An information theoretic model for summarization, and some basic results

A basic information theoretic model for summarization is formulated. Here summarization is considered as the process of taking a report of $v$ binary objects, and producing from it a $j$ element subset that captures most of the important features of the original report, with importance being defined via an arbitrary set function endemic to the model. The loss of information is then measured by a weight average of variational distances, which we term the semantic loss. Our results include both cases where the probability distribution generating the $v$-length reports are known and unknown. In the case where it is known, our results demonstrate how to construct summarizers which minimize the semantic loss. For the case where the probability distribution is unknown, we show how to construct summarizers whose semantic loss when averaged uniformly over all possible distribution converges to the minimum.

==> proofs.tex <==

\section{Proofs}

\subsection{Theorem~\ref{thm:optimal_known_p}}
\begin{IEEEproof}
First observe that 
\begin{align}
    \mathbb{D}_{f}(1_{x} || i_{y})  = f(0) + i_{y}(x) \left[ f\left( \frac{1}{i_y(x)} \right) - f(0) \right] \label{eq:thm3:obs1}
\end{align}
since 
\begin{align*}
\mathbb{D}_{f}(1_{x} || i_{y}) &= \sum_{\tilde x} i_{y}(\tilde x) f\left( \frac{1_{x}(\tilde x)}{i_{y}(\tilde x)} \right) \\
&= i_{y}(x) f \left( \frac{1}{i_y(x)} \right) + \sum_{\tilde x \neq x} i_{y}(\tilde x) f\left( \frac{0}{i_{y}(\tilde x)} \right)  \\
&= i_{y}(x) f \left( \frac{1}{i_y(x)} \right) + \left[ 1 -i_{y}( x) \right] f\left(0 \right)  \\
&= f(0) + i_{y}(x) \left[ f\left( \frac{1}{i_y(x)} \right) - f(0) \right].
\end{align*}
From this observation follows that $\mathbb{D}_{f}(1_{x}||i_y)$ is non-increasing as $i_{y}(x)$ increases. Indeed,
\begin{align}
\frac{\dx}{\dx u} f(0) + u^{-1} \left[ f\left( u \right) - f(0)\right] &= - u^{-1} \left[ \frac{f(u) - f(0)}{u} -  f'(u) \right] 
\end{align}
and hence there exists a $\zeta \in [0, u]$ such that 
\begin{align}
\frac{\dx}{\dx u} f(0) + u^{-1} \left[ f\left( u \right) - f(0)\right] &= -u^{-1} \left[ f'(\zeta) - f'(u) \right] 
\end{align}
by the mean value theorem. But $$ f'(\zeta) - f'(u) \leq 0  $$  since $\zeta \leq u$ and $f$ is a convex function. Therefore we have that 
$$\frac{\dx}{\dx u} f(0) + u^{-1} \left[ f\left( u \right) - f(0)\right] \geq 0 $$
for all $u \geq 0$, which in turn implies that if $u \geq w $ then 
\begin{align}
f(0) + u^{-1} \left[ f\left( u \right) - f(0)\right] \geq f(0) + w^{-1} \left[ f\left( w \right) - f(0) \right]. \label{eq:thm3:ineq2}
\end{align}
Hence for $y,\tilde y \in 2^{\mcf{V}}$, where $i_{y}(x)  \geq i_{\tilde y}(x) $,
\begin{align}
\mathbb{D}_{f}(1_{x} || i_{y}) &= f(0)+ i_{y}(x) \left[ f\left( \frac{1}{i_y(x)} \right) - f(0) \right] \\
&\leq f(0) + i_{\tilde y}(x) \left[ f\left( \frac{1}{i_{\tilde y}(x)} \right) - f(0) \right] = \mathbb{D}_{f}(1_{x} || i_{\tilde y}) \label{eq:thm3:obs2}
\end{align}
follows by two applications of Equation~\eqref{eq:thm3:obs1} and setting $u = \frac{1}{i_{\tilde y}(x)}$ and $w = \frac{1}{i_{y}(x)}$ in Equation~\eqref{eq:thm3:ineq2}.

From Equation~\eqref{eq:thm3:obs2} we can now finish the proof of the theorem. To do this suppose that there was a summarizer $s \in \mcf{P}(2^{\mcf{V}}|(2^{\mcf{V}})^{\otimes n + 1})$ 
such that
$$s_{x,\hat x^n}(y) > 0 \text{ only if } y \in \mcf{Y}^{(i,j)}(x) $$
for each $(x,\hat x^n,y)$
which did not achieve the minimum $c$. In this case there must exist a summarizer $q \in \mcf{P}(2^{\mcf{V}}|(2^{\mcf{V}})^{\otimes n + 1})$
such that 
\begin{align}
\sum_{x,\hat x^n, y} p(x) \hat p_{x}(\hat x^n) s_{x,\hat x^n}(y) \mathbb{D}(1_{x}||i_{y}) - \sum_{x,\hat x^n, z} p(x)\hat p_{\hat x}(x^n) q_{x,\hat x^n}(z) \mathbb{D}(1_{x}||i_{z})> 0 .
\end{align}
This leads to a contradiction though since
\begin{align}
\sum_{x,\hat x^n, y} p(x) \hat p_{x}(\hat x^n) s_{x,\hat x^n}(y) \mathbb{D}(1_{x}||i_{y}) &=  \sum_{x,\hat x^n} p(x) \hat p_{x}(\hat x^n) \min_{y : x \in 2^{\mcf{V}}(y), |y| \leq j}  \mathbb{D}(1_{x}||i_{y})\\
&=  \sum_{x,\hat x^n,z} p(x) \hat p_{x}(\hat x^n) q_{x,\hat x^n}(z) \min_{y : x \in 2^{\mcf{V}}(y), |y| \leq j}  \mathbb{D}(1_{x}||i_{y}) \\ 
&\leq  \sum_{x,\hat x^n,z} p(x) \hat p_{x}(\hat x^n) q_{x,\hat x^n}(z)  \mathbb{D}(1_{x}||i_{z}).
\end{align}


\end{IEEEproof}

\subsection{Theorem~\ref{thm:4}}


%$\prescript{14}{2}{k}$
Begin by expressing the semantic loss ensemble as 
%\begin{align}
%-\int_{\mcf{P}(\mcf{X})} \sum_{\hat x^n, x , y } s_{x, \hat x^n}(y)  \Pr\left(\hat X^n = \hat x^n, X =  x \middle| P=p \right)  \ln a_{y}(x) \dx p %\label{eq:proof:KL|PU}
%\end{align}
\begin{align}
 \sum_{\substack{\hat x^n \in \mcf{X}^{n},\\ x \in \mcf{X}  ,\\ y \in \mcf{Y} , \\ z \in \mcf{Z}, \\  \mcf{W}\subseteq \mcf{X}} } u(x,\mcf{W}) s_{x, \hat x^n}(y,z) \int_{\mcf{P}(\mcf{X})}   p(x) \left( \prod_{\tilde x \in \mcf{X} } p(\tilde x)^{ n\pi^{(\hat x^n)}(\tilde x)} \right) g(p) \left[ f(0)+ i_{y,z}(\mcf{W}) \left[ f \left( \frac{1}{i_{y,z}(\mcf{W})} \right) - f(0) \right] \right] \dx p \label{eq:proof:KL|PU}
\end{align}
where $g$ is a uniform probability density function over $\mcf{P}(\mcf{X})$. 
%Indeed $$\ell(X;Y,a) = \mathbb{E}\left[ \mathbb{D}_{f}(1_{\{X\}}|| a_{Y}) \right] = \mathbb{E} \left[ \mathbb{E}\left[ \mathbb{D}_{f}(1_{\{X\}}|| a_{Y}) \middle| \hat X^n, P \right]  \right],$$ while $\hat X^n, X$ is a collection of $n+1$ IID random variables once given the distribution $p$. 
From here the goal is to determine
\begin{align}
% \sum_{\mcf{W} \subseteq \mcf{X}} u(x,\mcf{W}) 
 \int_{\mcf{P}(\mcf{X})}  p(x) \left( \prod_{\tilde x \in \mcf{X} } p(\tilde x)^{ n\pi^{(\hat x^n)}(\tilde x)} \right)  g(p) \frac{p(\mcf{W} \cap \mcf{X}(y,z))}{p(\mcf{X}(y,z))} \left[ f \left( \frac{p(\mcf{X}(y,z))}{p(\mcf{W} \cap \mcf{X}(y,z))} \right) - f(0) \right]  \dx p   \label{eq:proof:goal},
\end{align}




To analyze~\eqref{eq:proof:goal}, let
\begin{align*}
p_{i} &\defn p(i) \\
\bar p_i &\defn 1 - \sum_{m=1}^{i-1} p_m \\
t_i &\defn  n\pi^{(\hat x^n)}(i)  \\
\bar t_i &\defn 2^{v} - i  + \sum_{m=i}^{2^v} t_m = 2^{v}-i + n - \sum_{m=1}^{i-1} t_m ,
\end{align*}
and without loss of generality assume that $x = 1$, $\mcf{X}(y,z) = \{1,\dots, 2^{v-j} = j^*\}$, and $\mcf{W}\cap \mcf{X}(y,z) = \{ 1, \dots,w \}$. Of importance throughout the proof will be that 
\begin{align}
\bar p_i = \bar p_{i-1} - p_{i-1} \label{eq:proof:helpful}
\end{align}
for all integers $i \in \{1,\dots, 2^{v}\},$ and that $\bar t_1 = n + 2^{v}-1$ and $\bar p_1 = 1$. These definitions will help in a recursive analysis. Indeed \eqref{eq:proof:goal} can be written
\begin{align}
& (2^v-1)! \int_{0}^{\bar p_1} \int_{0}^{\bar p_2} \dots \int_{0}^{\bar p_{2^v-1}} p_1^{1+t_1} \left( \prod_{m=2}^{2^v-2} p_m^{t_m} \right)\frac{\sum_{m=1}^w p_m }{\sum_{m=1}^{j^*} p_m} \left[ f \left( \frac{\sum_{m=1}^{j^*} p_m}{\sum_{m=1}^w p_m } \right) - f(0) \right]  \notag \\
&\hspace{15pt} \cdot \int_{0}^{\bar p_{2^v-1}}  p_{2^v-1}^{t_{2^v-1}} \left( \bar p_{2^{v}-1} - p_{2^v-1}\right)^{t_{2^v}}  ~\dx p_{2^v-1} \dots \dx p_{1} \label{eq:proof:m-1}
\end{align}
by recognizing that
$$\mcf{P}(\mcf{X}) = \set{ (p_1,\dots,p_{|\mcf{X}|}) \in \mathbb{R}^{|\mcf{X}|} : \left( \begin{array}{l}  p_i \in \left[ 0, \bar p_i \right] \\ ~~~~i \in \set{1,\dots,|\mcf{X}|-1},\\ p_{|\mcf{X}|} =  \bar p_{|\mcf{X}|}  \end{array} \right) } ,$$
and then making use of Corollary~\ref{cor:proof:ok} and Equation~\eqref{eq:proof:helpful}. 
Performing the first integration of~\eqref{eq:proof:m-1} (via Lemma~\ref{lem:proof:ok}) then yields
\begin{align}
& (2^v-1)! \frac{t_{2^v}! t_{2^v-1}!}{\bar t_{2^v-1}!} \int_{0}^{\bar p_1} \int_{0}^{\bar p_2} \dots \int_{0}^{\bar p_{2^v-3}} p_1^{1+t_1} \left( \prod_{m=2}^{2^v-3} p_m^{t_m} \right) \frac{\sum_{m=1}^w p_m }{\sum_{m=1}^{j^*} p_m} \left[ f \left( \frac{\sum_{m=1}^{j^*} p_m}{\sum_{m=1}^w p_m } \right) - f(0) \right]  \notag \\
&\hspace{15pt} \cdot \int_{0}^{\bar p_{2^v-2}}  p_{2^v-2}^{t_{2^v-2}} \left( \bar p_{2^{v}-2} - p_{2^v-2}\right)^{t_{2^v-1}}  ~\dx p_{2^v-2} \dots \dx p_{1}   \label{eq:proof:m-2}
\end{align}
where Equation~\eqref{eq:proof:helpful} is used to obtain the $\bar p_{2^{v}-2} - p_{2^{v}-2}$ term.
At this point it is important to recognize that~\eqref{eq:proof:m-2} is only superficially different than~\eqref{eq:proof:m-1}, and that the same integration may repeated to evaluate the integrals over $p_{2^v-2},\dots,p_{2^{v-j}+1}$; doing so yields
\begin{align}
&\frac{  (2^v-1)! \prod_{m=j^*+1}^{2^v} t_m! }{\bar t_{j^*+1} !}  \int_{0}^{\bar p_1} \dots \int_{0}^{\bar p_{j^*} }p_1^{1+t_1} \left( \prod_{m=2}^{j^*-1} p_m^{t_m} \right) \notag\\
&\hspace{40pt} \cdot p_{j^*}^{t_{j^*}}  \left(\bar p_{j^*} - p_{j^*} \right)^{\bar t_{j^*+1}} \frac{\sum_{m=1}^w p_m }{\sum_{m=1}^{j^*} p_m} \left[ f \left( \frac{\sum_{m=1}^{j^*} p_m}{\sum_{m=1}^w p_m } \right) - f(0) \right]  ~\dx p_{j^*} \dots \dx p_{1}
\label{eq:proof:ell}.
\end{align}

At this point the recursion no longer directly applies since the next variable of integration, $p_{2^{v-j}}$, is contained inside the logarithm. 
To address this, use the Taylor series expansion\footnote{This continues to hold when $\sum_{m=1}^w p_m = 0$ since $0 \ln 0  = 0 $ by definition. On the other hand, to check the RHS of Equation~\eqref{eq:proof:taylor} is $0$ observe that $p_{2^{v-j}} \leq \bar p_{2^{v-j}}  \leq \bar p_w - p_w \leq 1 - p_1 $ implies the RHS of~\eqref{eq:proof:taylor} is not negative and that it must be less than $p_1 \sum_{k=1}^\infty \frac{(1-p_1)^k}{k} = \sum_{k=1}^\infty \frac{(1-p_1)^k - (1-p_1)^{k+1}}{k} = \sum_{k=1}^\infty \frac{(1-p_1)^k}{k} - \frac{(1-p_1)^{k+1}}{k+1} -  \sum_{k=1}^\infty (1-p_1)^{k+1} \left[ \frac{1}{k} - \frac{1}{k+1} \right] = 0 $. } of $\ln (1 - x)$, specifically as follows
\begin{align} 
p_1 \ln \frac{\sum_{m=1}^{2^{v-j}} p_m}{\sum_{m=1}^w p_m} 
&= p_1 \ln ( 1- (\bar p_{2^{v-j}} - p_{2^{v-j}}) ) - p_1 \ln ( 1 -(\bar p_w - p_w)) \notag \\
&= -p_1 \sum_{k=1}^\infty \frac{(\bar p_{2^{v-j}} - p_{2^{v-j}})^k}{k}  + p_1 \sum_{k=1}^\infty \frac{(\bar p_w - p_w)^k}{k} . \label{eq:proof:taylor} 
\end{align}
Plugging~\eqref{eq:proof:taylor} into~\eqref{eq:proof:ell} and exchanging the summations and integrals results in
\begin{align}
&\frac{  (2^v-1)! \prod_{m=2^{v-j}+1}^{2^v} t_j! }{\bar t_{2^{v-j}+1}!} \sum_{k=1}^\infty \frac{1}{k}  \notag \\
&\hspace{30pt} \cdot \left[  - \int_{0}^{\bar p_1} \dots \int_{0}^{\bar p_{2^{v-j}}} p_1^{1+t_1} \left( \prod_{m=2}^{2^{v-j}-1} p_m^{t_m} \right) p_{2^{v-j}}^{t_{2^{v-j}}}  \left(\bar p_{2^{v-j}} - p_{2^{v-j}}\right)^{\bar t_{2^{v-j}+1} + k } ~\dx p_{2^{v-j}} \dots \dx p_{1} \right. \notag \\
& \hspace{30pt} \left.  +  \int_{0}^{\bar p_1} \dots \int_{0}^{\bar p_{2^{v-j}}} p_1^{1+t_1}(\bar p_w - p_w)^{k} \left( \prod_{m=2}^{2^{v-j}-1} p_m^{t_m} \right) p_{2^{v-j}}^{t_{2^{v-j}}}  \left(\bar p_{2^{v-j}} - p_{2^{v-j}}\right)^{\bar t_{2^{v-j}+1} } ~\dx p_{2^{v-j}} \dots \dx p_{1}  \right]
\label{eq:proof:ellk}.
\end{align}
Once again recognize that both integrals in~\eqref{eq:proof:ellk} are only superficially different to those of~\eqref{eq:proof:m-1}, and hence we can apply the same recursive analysis as before; integrating over variables $p_{2^{v-j}},\dots, p_2$ yields 
\begin{align}
&\sum_{k=1}^{\infty} \frac{1}{k} \frac{  (2^v-1)! \prod_{m=2}^{2^v} t_m! }{\bar t _{2^{v-j}+1} !}  \left[ \frac{\bar t _{2^{v-j}+1} ! (\bar t_{w+1}+ k)!}{\bar t_{w+1}! (\bar t_2 + k) !} - \frac{(\bar t _{2^{v-j}+1}  + k)!}{(\bar t _{2}+ k)!} \right] \int_{0}^{\bar p_1} p_1^{1+t_1} \left( \bar p_1 - p_1 \right)^{\bar t_{2} + k}  \dx p_{1} 
\label{eq:proof:ellk2},
\end{align}
and then integrating over $p_1$ and simplifying gives
\begin{align}
&\sum_{k=1}^{\infty} \frac{t_1 + 1 }{k} \frac{  (2^v-1)! \prod_{m=1}^{2^v} t_m! }{(\bar t_1 + 1  + k)!}   \left[ \frac{ (\bar t_{w+1}+k)!}{\bar t_{w+1}!} - \frac{(\bar t_{2^{v-j}+1}+k)!}{\bar t_{2^{v-j}+1}!} \right].
\end{align}
Replacing the $t$ and $\bar t$ terms with their original meanings yields
\begin{align}
&\sum_{k=1}^{\infty} \frac{n \pi^{(\hat x^n)}(x) + 1 }{k} \frac{  (2^v-1)! \prod_{\tilde x \in \mcf{X}} (n \pi^{(\hat x^n)}(\tilde x))! }{(n + 2^{v} + k)!}   
\left[ \zeta_{k,1}(\mcf{W}\cap \mcf{X}(y,z)) - \zeta_{k,1}(\mcf{X}(y,z) ) \right]
%\left[ \frac{(n-\sum_{m=1}^w t_m + 2^v - (w+1) + k)!}{(n-\sum_{m=1}^w t_m  + 2^v - (w+1) )! } - \frac{(n - \sum_{m=1}^{2^{v-j}} t_m + 2^v - (2^{v-j} + 1) + k)!}{(n - \sum_{m=1}^{2^{v-j}} t_m + 2^v - (2^{v-j}+1))!} \right]
\label{eq:proof:ellk3},
\end{align}
where 
$$ \zeta_{k,a}( \mcf{\hat X} ) = \zeta_{k,a}(\mcf{\hat X}|\hat x^n) \defn \frac{(n- \sum_{\tilde x \in \mcf{\hat X}} n \pi^{(\hat x^n)}(\tilde x) + 2^v - (|\mcf{\hat X}|+a) + k)!  }{(n- \sum_{\tilde x \in \mcf{\hat X}} n \pi^{(\hat x^n)}(\tilde x) + 2^v - (|\mcf{\hat X}|+a))!} $$
for $\mcf{\hat X} \subseteq \mcf{X}$ and integers $a$ and $k$.
Equation~\eqref{eq:proof:ellk3} can now be plugged back into Equation~\eqref{eq:proof:KL|PU}, and the average semantic loss written as the uniform average over all possible empirical distributions of $\hat x^n,$ where each sequence is equally likely given said distribution, and $x$ is distributed according to a weighted distribution. In specific
\begin{align}
&\sum_{\hat x^n \in \mcf{X}^n} \frac{(2^v-1)! n!}{(n+2^v-1)!} \frac{\prod_{\tilde x \in \mcf{X}} (n \pi^{(\hat x^n)}(\tilde x))!}{n!} \sum_{x \in \mcf{X}} \frac{n \pi^{(\hat x^n)}(x) + 1 }{n+2^v} \sum_{\substack{y \in \mcf{Y}\\ z \in \mcf{Z}}} s_{x,\hat x^n}(y,z)  \notag \\
&\hspace{20pt} \cdot \sum_{ \mcf{W} \subseteq \mcf{X}}  u(x, \mcf{W})  \sum_{k=1}^{\infty}     \frac{ \zeta_{k,1}(\mcf{W} \cap \mcf{X}(y,z)|\hat x^n) - \zeta_{k,1}(\mcf{X}(y,z) |\hat x^n)}{k \zeta_{k,0}(\emptyset) }.
\end{align}
This is indeed an average, since $\frac{(n+2^v-1)!} {(2^v-1)!n!}$ is the total number of possible empirical distributions distributions for $n$ symbols chosen from a $2^v$-size alphabet, while $\frac{n!}{\prod_{\tilde x \in \mcf{X}} (n \pi^{(\hat x^n)}(\tilde x))!}$ is the total number of distinct $n$-symbol sequences for a particular empirical distribution, and finally $\frac{n \pi^{(\hat x^n)}(x) + 1 }{n+2^v}$ is a valid probability density function since the sum is $1$ and each term is positive.

\textcolor{green}{To prove Theorem~\ref{thm:4} consider that the value of $t_1 = \pi_{\hat x^n}(x)$ will be fixed regardless of the summary chosen, while on the other hand
$$ \frac{(b+k)!}{b!} = (b+1)\cdot\dots\cdot (b+k) < (b+c+1) \cdot \dots \cdot (b+c+k) = \frac{(b+c+k)!}{(b+c)!}$$
for all positive integers $b,c: b<c$ and $k$. 
Recall then that
$$\sum_{m=1}^{2^{v-j}} t_m = n\sum_{\tilde x \in 2^{\mcf{V}}(y)}  \pi^{(\hat x^n)}(\tilde x), $$
from which it now follows that~\eqref{eq:proof:goal} must monotonically increase as $\sum_{\tilde x \in 2^{\mcf{V}}(y)}  \pi^{(\hat x^n)}(\tilde x)$ increases.}


==> proofs_old.tex <==



\subsection{Theorem~\ref{lem:some_lb}}\label{sec:some_lb}

\begin{IEEEproof}
The theorem follows directly from Lemma~\ref{lem:thistooktoolong}.
\end{IEEEproof}




==> scrap.tex <==



Using Robbins' sharpening of Stirling's formula for the factorials gives
\begin{align}
\frac{a!}{(a+k)!} &\approx \frac{a^{a+\frac{1}{2}} e^{-a}}{(a+k)^{a+k+ \frac{1}{2}} e^{-a-k}}= \left( \frac{a}{a+k }\right)^{a+k+ \frac{1}{2}} \left(\frac{e}{a}\right)^{k}
\end{align}


\begin{align}
\frac{(x+k)!}{x!} &\approx x^k \left( \left[ 1+ \frac{k}{x} \right]^{x+k+1/2} e^{-k} \right)\\
&= \left(\frac{e k}{x} \right)^{x+1/2} e^{-k - 1/2} k^k  \left( \left[ 1+ \frac{x}{k} \right]^{x+k+1/2} e^{-x} \right)
\end{align}



\begin{align}
\frac{a!(b+k)!}{(a+k)!b!} &= \left( \frac{b}{a} \right)^k \frac{\left( 1 + \frac{k}{b} \right)^{b+k+1/2}}{\left( 1 + \frac{k}{a} \right)^{a+k+1/2}}\\
&= \left( \frac{a^{a+1/2}}{b^{b+1/2}} (ek)^{b-a} \right)  \left[\frac{e^{-b} \left( 1 + \frac{b}{k} \right)^{b+k+1/2} }{e^{-a}\left( 1 + \frac{a}{k} \right)^{a+k+1/2} } \right]
\end{align}

Multiplicative error for 1/1-
$$ \frac{ \left( 1+\frac{k}{b} \right)^{b+k+1/2} }{\left( 1 + \frac{k}{a} \right)^{a+k+1/2} }  $$
which converges to $1$ with $b$ if $k < \frac{\sqrt{b}}{\ln b}$ and $a = \chi b$, otherwise if $b$ is arbitrary close to $a$, then $k$ may be allowed to go as large as $b$.


\noindent 2/1-
$$ \frac{ \left( 1+\frac{b}{k} \right)^{b+k+1/2} e^{-b} }{\left( 1 + \frac{k}{a} \right)^{a+k+1/2} e^{-k} }  $$
2/2-
$$ \frac{ \left( 1+\frac{b}{k} \right)^{b+k+1/2} e^{-b} }{\left( 1 + \frac{a}{k} \right)^{a+k+1/2} e^{-a} }  \leq 1  $$

%\begin{align*} \frac{ \left( 1+\frac{b}{k} \right)^{b+k+1/2} e^{-b} }{\left( 1 + \frac{a}{k} \right)^{a+k+1/2} e^{-a} }  &= \sqrt{\frac{b+k}{a+k}} e^{a -b + \left(b+k\right)\ln \left( 1 + \frac{b}{k}\right) -\left(a+k\right)\ln \left(1 + \frac{a}{k} \right)} \\
%&\leq \sqrt{\frac{b+k}{a+k}} e^{a -b + \left(b+k\right)\left(\frac{b}{k} - \frac{b^2}{2k^2} + \frac{b^3}{3k^3} \right) -\left(a+k\right)\left(\frac{a}{k} - \frac{a^2}{2k^2}\right)} \\
%&=\sqrt{\frac{b+k}{a+k}} e^{a -b + \frac{b^2}{k} - \frac{b^3}{2k^2} + \frac{b^4}{3k^3} +b - \frac{b^2}{2k} + \frac{b^3}{3k^2} - \frac{a^2}{k} - a  + \frac{a^3}{2k^2} + \frac{a^2}{2k}  } \\
%&= \sqrt{\frac{b+k}{a+k}} e^{\frac{b^2-a^2}{2k} + \frac{3 a^3 - b^3 }{6k^2} + \frac{b^4}{3k^3} }
%\end{align*}

Approximation for 1/1-
$$\left(  \frac{b}{a}\right)^k$$
2/1-
$$ \frac{\left( \frac{e k}{b} \right)^{b+1/2} e^{-k - 1/2} k^k  }{a^k} = \left( \frac{e k}{b} \right)^{b} \left(\frac{k}{ea} \right)^{k} \sqrt{\frac{k}{b}}  $$ 
2/2-
$$ \left(\frac{e k}{b} \right)^{b+1/2} \left(\frac{a}{e k} \right)^{a+1/2} = \frac{a^{a+1/2}}{b^{b+1/2}} (ek)^{b-a} $$


$$\frac{\dx}{\dx k} \left( 1 + \frac{k}{a} \right)^{a+k+1/2} = \left[ \ln \left( 1 + \frac{k}{a} \right) + 1 + \frac{1}{2(a+k)} \right] \left( 1 + \frac{k}{a} \right)^{a+k+1/2} $$




\begin{align*}
\frac{\dx}{\dx x} \left( 1 + \frac{k}{x} \right)^{k+x+\frac{1}{2}} &= \left( 1 + \frac{k}{x} \right)^{k+x+\frac{1}{2}} \left[ \ln \left( 1 + \frac{k}{x} \right) - \frac{k}{x} \left( 1 + \frac{1}{2(k+x)} \right) \right] \leq 0
\end{align*}

$$ \left( 1 + \frac{k}{x} \right)^{k+x+\frac{1}{2}} \searrow_{x} e^{k} $$

\begin{align*}
    \frac{\dx}{\dx x} \left( \frac{x}{b}\right)^k \left( \frac{\left(1+ \frac{k}{x}\right)^{k+x+\frac{1}{2}} }{\left( 1 +\frac{k}{c}\right)^{k+ c+ \frac{1}{2} }} - 1 \right) &= \frac{x^{k-1}}{b^k}\left( \frac{\left(1+ \frac{k}{x}\right)^{k+x+\frac{1}{2}} }{\left( 1 +\frac{k}{c}\right)^{k+ c+ \frac{1}{2} }} \left[ k + x \ln \left( 1 + \frac{k}{x} \right) -k -\frac{k}{2(k+x)} \right] - k \right) \\
    &=\frac{x^{k-1}}{b^k}\left( \frac{\left(1+ \frac{k}{x}\right)^{k+x+\frac{1}{2}} }{\left( 1 +\frac{k}{c}\right)^{k+ c+ \frac{1}{2} }} \left[  x \ln \left( 1 + \frac{k}{x} \right)  -\frac{k}{2(k+x)} \right] - k \right) \\
    &=\frac{x^{k-1}}{b^k \left( 1 +\frac{k}{c}\right)^{k+ c+ \frac{1}{2} } }\left( \left(1+ \frac{k}{x}\right)^{k+x+\frac{1}{2}}  \left[  x \ln \left( 1 + \frac{k}{x} \right)  -\frac{k}{2(k+x)} \right] -  \left( 1 +\frac{k}{c}\right)^{k+ c+ \frac{1}{2} } k \right) 
\end{align*}


\begin{align*}
    \frac{\dx}{\dx k} \frac{\left( 1 + \frac{k}{b} \right)^{b+k+1/2}}{\left( 1 + \frac{k}{c} \right)^{c+k+1/2}} &= \frac{\left( 1 + \frac{k}{b} \right)^{b+k+1/2}}{\left( 1 + \frac{k}{c} \right)^{c+k+1/2}} \left[ \ln\left( 1 + \frac{k}{b} \right) + \frac{k + b + \frac{1}{2}}{k+b}  - \ln\left( 1 + \frac{k}{c} \right) - \frac{k + c + \frac{1}{2}}{k+c}  \right]\\
    &= \frac{\left( 1 + \frac{k}{b} \right)^{b+k+1/2}}{\left( 1 + \frac{k}{c} \right)^{c+k+1/2}} \left[ \ln\left( \frac{1 + \frac{k}{b}}{1 + \frac{k}{c}} \right) + \frac{1}{2(k+b)} - \frac{1}{2(k+c)}  \right]\\
    &= \frac{\left( 1 + \frac{k}{b} \right)^{b+k+1/2}}{\left( 1 + \frac{k}{c} \right)^{c+k+1/2}} \left[ \ln\left( \frac{1 + \frac{k}{b}}{1 + \frac{k}{c}} \right) + \frac{c-b}{2(k+b)(k+c)}   \right]
\end{align*}

\begin{align*}
&\frac{\dx}{\dx k} \frac{1}{k} \left( \frac{x}{b}\right)^k \left( \frac{\left(1+ \frac{k}{x}\right)^{k+x+\frac{1}{2}} }{\left( 1 +\frac{k}{c}\right)^{k+ c+ \frac{1}{2} }} - 1 \right) \\
&= \frac{-1}{k^2} \left( \frac{x}{b}\right)^k \left( \frac{\left(1+ \frac{k}{x}\right)^{k+x+\frac{1}{2}} }{\left( 1 +\frac{k}{c}\right)^{k+ c+ \frac{1}{2} }} - 1 \right) +\ln \left( \frac{x}{b} \right) \frac{1}{k} \left( \frac{x}{b}\right)^k \left( \frac{\left(1+ \frac{k}{x}\right)^{k+x+\frac{1}{2}} }{\left( 1 +\frac{k}{c}\right)^{k+ c+ \frac{1}{2} }} - 1 \right) \\
&\hspace{10pt} + \frac{1}{k} \left( \frac{x}{b}\right)^k \frac{\left( 1 + \frac{k}{x} \right)^{x+k+1/2}}{\left( 1 + \frac{k}{c} \right)^{c+k+1/2}} \left[ \ln\left( \frac{1 + \frac{k}{x}}{1 + \frac{k}{c}} \right) + \frac{c-x}{2(k+x)(k+c)}   \right] \\
&= \frac{1}{k} \left( \frac{x}{b}\right)^k \left[ \left( \frac{-1}{k} + \ln \left( \frac{x}{b} \right) + \ln\left( \frac{1 + \frac{k}{x}}{1 + \frac{k}{c}} \right) + \frac{c-x}{2(k+x)(k+c)}  \right)\left( \frac{\left(1+ \frac{k}{x}\right)^{k+x+\frac{1}{2}} }{\left( 1 +\frac{k}{c}\right)^{k+ c+ \frac{1}{2} }} - 1 \right)  \right.\\
&\hspace{10pt} \left. + \ln\left( \frac{1 + \frac{k}{x}}{1 + \frac{k}{c}} \right) + \frac{c-x}{2(k+x)(k+c)} \right]\\
&= \frac{1}{k} \left( \frac{x}{b}\right)^k \left[ \left( \frac{-1}{k} + \ln \left( \frac{c}{b} \right) + \ln\left( 1 - \frac{c-x}{c+k}  \right) + \frac{c-x}{2(k+x)(k+c)}  \right)\left( \frac{\left(1+ \frac{k}{x}\right)^{k+x+\frac{1}{2}} }{\left( 1 +\frac{k}{c}\right)^{k+ c+ \frac{1}{2} }} - 1 \right)  \right.\\
&\hspace{10pt} \left. + \ln\left( \frac{1 + \frac{k}{x}}{1 + \frac{k}{c}} \right) + \frac{c-x}{2(k+x)(k+c)} \right]
\end{align*}



\begin{align*}
\frac{\dx}{\dx k} \left( \frac{a}{b}\right)^k  \frac{\left(1+ \frac{k}{a}\right)^{k+a+\frac{1}{2}} }{\left( 1 +\frac{k}{b}\right)^{k+ b+ \frac{1}{2} }}  &= \left( \frac{a}{b}\right)^k  \frac{\left(1+ \frac{k}{a}\right)^{k+a+\frac{1}{2}} }{\left( 1 +\frac{k}{b}\right)^{k+ b+ \frac{1}{2} }} \left[ \ln \left( 1 - \frac{b-a}{b+k} \right) + \frac{b-a}{2(b+k)(a+k)} \right] \leq 0 
\end{align*}



\begin{align*}
\frac{\dx}{\dx k} \left( \frac{a}{b}\right)^k \left( \frac{\left(1+ \frac{k}{a}\right)^{k+a+\frac{1}{2}} }{\left( 1 +\frac{k}{c}\right)^{k+ c+ \frac{1}{2} }} -1 \right) &= \left( \frac{a}{b}\right)^k  \left[ \frac{\left(1+ \frac{k}{a}\right)^{k+a+\frac{1}{2}} }{\left( 1 +\frac{k}{c}\right)^{k+ c+ \frac{1}{2} }} \left( \ln \left(\frac{c}{b} \right) + \ln \left( 1 - \frac{c-a}{c+k} \right) + \frac{c-a}{2(c+k)(a+k)} \right) + \ln\left( \frac{b}{a} \right) \right]  
\end{align*}


\begin{align*}
\sum_{j = \tilde k + 1 }^\infty\frac{1}{j}  \frac{a^{a+\frac{1}{2}}}{b^{b+\frac{1}{2}}} \frac{1}{e^{a-b}}  j^{-(a-b)}
&\leq \frac{a^{a+\frac{1}{2}}}{b^{b+\frac{1}{2}}} \frac{1}{e^{a-b}}  \frac{1}{(a-b) \tilde k^{a-b}}\\
&= \sqrt{\frac{1}{\rho}} \left(\frac{1}{\rho} \right)^{a \rho} \left( \frac{a}{e \tilde k} \right)^{a(1-\rho)} \frac{1}{a(1-\rho)}
\end{align*}


\begin{align*}
\frac{\dx}{\dx \rho} \sqrt{\frac{1}{\rho}} \left(\frac{1}{\rho} \right)^{a \rho} \left( \frac{a}{e \tilde k} \right)^{a(1-\rho)} \frac{1}{a(1-\rho)} 
&= \sqrt{\frac{1}{\rho}} \left(\frac{1}{\rho} \right)^{a \rho} \left( \frac{a}{e \tilde k} \right)^{a(1-\rho)} \frac{1}{a(1-\rho)}  \left[\frac{-1}{2\rho} + \frac{1}{1-\rho} + a \ln \left( \frac{1}{\rho} \right)  -a - a \ln \left( \frac{a}{e\tilde k} \right)    \right] \\
&= \sqrt{\frac{1}{\rho}} \left(\frac{1}{\rho} \right)^{a \rho} \left( \frac{a}{e \tilde k} \right)^{a(1-\rho)} \frac{1}{a(1-\rho)}  \left[\frac{-1}{2\rho} + \frac{1}{1-\rho} + a \ln \left( \frac{\tilde k}{a \rho} \right)     \right] 
\end{align*}

The maximums of the above occur at $\rho  = 0 , 1$ and $\rho \approx \frac{\tilde k}{a}$. 


\begin{align*}
\lim_{\rho \rightarrow 0^+} \sqrt{\frac{1}{\rho}} \left(\frac{1}{\rho} \right)^{a \rho} \left( \frac{a}{e \tilde k} \right)^{a(1-\rho)} \frac{1}{a(1-\rho)} &= \sqrt{\frac{1}{0}} 1 \left( \frac{a}{e\tilde k} \right)^a \frac{1}{a}   = \infty\\
\lim_{\rho \rightarrow 1^+} \sqrt{\frac{1}{\rho}} \left(\frac{1}{\rho} \right)^{a \rho} \left( \frac{a}{e \tilde k} \right)^{a(1-\rho)} \frac{1}{a(1-\rho)} &= \sqrt{\frac{1}{1}}  \frac{1}{0}   = \infty
\end{align*}

The solution to this problem is to set $\tilde k$ equal to $a$, and thus $\rho = 1 - \frac{2}{a}$ becomes the one and only maximum. This is only really necessary I think if $\rho$



At $k=\mu a$, for positive rational number $\mu$,
\begin{align*}
\frac{a^{a+k+1/2}}{b^{b+k+1/2}} \frac{ (b+k)^{b+k+1/2}}{(a+k)^{a+k+1/2}} e^{-k\epsilon } & = \left( \frac{\rho + \mu}{\rho} \right)^{(\rho+\mu) a + \frac{1}{2}} \left( \frac{1}{1+\mu} \right)^{(1+\mu) a + \frac{1}{2}} e^{-\mu a \epsilon} \\
&= \exp \left\{ \frac{\epsilon}{2} +   \rho a  \ln \left(1 + \frac{\mu}{\rho}  \right)  - a   \ln (1 + \mu) + \left(  \mu a + \frac{1}{2} \right) \left[ \ln \left( \frac{1+ \frac{\mu}{\rho}}{1 +\mu} \right) - \epsilon \right]  \right\}\\
&= \exp \left\{ \frac{\epsilon}{2} +   a  \ln \left[ \frac{\left(1 + \frac{\mu}{\rho}  \right)^\rho}{1+\mu } \right]+ \left(  \mu a + \frac{1}{2} \right) \left[ \ln \left( \frac{1+ \frac{\mu}{\rho}}{1 +\mu} \right) - \epsilon \right]  \right\}\\
%&= \exp \left\{ \left( \rho a + \frac{1}{2} \right) \epsilon   - \left( 1 -\rho \right) a  \ln (1 + \mu) + \left(\mu a  + \rho a + \frac{1}{2}\right) \left[ \ln \left( \frac{1+ \frac{\mu}{\rho}}{1 +\mu} \right) - \epsilon \right]  \right\}
\end{align*}

(change to a multiplier of $e^{\epsilon/2}$ on the whole thing, at $k=\mu a$, for positive rational number $\mu$,
\begin{align*}
\frac{a^{a+k+1/2}}{b^{b+k+1/2}} \frac{ (b+k)^{b+k+1/2}}{(a+k)^{a+k+1/2}} e^{-(k+1/2)\epsilon } & = \left( \frac{\rho + \mu}{\rho} \right)^{(\rho+\mu) a + \frac{1}{2}} \left( \frac{1}{1+\mu} \right)^{(1+\mu) a + \frac{1}{2}} e^{-(\mu a + 1/2) \epsilon} \\
&= \exp \left\{  \rho a  \ln \left(1 + \frac{\mu}{\rho}  \right)  - a   \ln (1 + \mu) + \left(  \mu a + \frac{1}{2} \right) \left[ \ln \left( \frac{1+ \frac{\mu}{\rho}}{1 +\mu} \right) - \epsilon \right]  \right\}\\
&= \exp \left\{    a  \ln \left[ \frac{\left(1 + \frac{\mu}{\rho}  \right)^\rho}{1+\mu } \right]+ \left(  \mu a + \frac{1}{2} \right) \left[ \ln \left( \frac{1+ \frac{\mu}{\rho}}{1 +\mu} \right) - \epsilon \right]  \right\}\\
&= \exp \left\{    a   \left( \ln \left[ \frac{\left(1 + \frac{\mu}{\rho}  \right)^\rho}{1+\mu } \right]+  \mu   \ln \left( \frac{1+ \frac{\mu}{\rho}}{1 +\mu} \right) -  \mu \epsilon  +  \frac{1}{2a } \left[ \ln \left( \frac{1+ \frac{\mu}{\rho}}{1 +\mu} \right) - \epsilon \right] \right)\right\}\\
&= \exp \left\{    a   \left( ( \rho + \mu) \ln \left( 1 + \frac{\mu}{\rho} \right) - (1+\mu) \ln \left( 1 + \mu \right) - \mu \epsilon   +  \frac{1}{2a } \left[ \ln \left( \frac{1+ \frac{\mu}{\rho}}{1 +\mu} \right) - \epsilon \right] \right)\right\}
\end{align*}


%y1 =  (u/v).^k .* ( 1+k/u).^(u+k+.5)./((1+k/v).^(v+k+.5)); y2 = (u/v).^k; y3 = (e*k/u).^u .* (k/(e*v)).^k .* (k/u ).^.5; y4 = v^(v+1/2)/(u^(u+1/2)) *(e*k).^(u-v);

